CriticEval: Evaluating Large Language Model as Critic

Critique ability, i.e., the capability of Large Language Models (LLMs) to identify and rectify flaws in responses, is crucial for their applications in self-improvement and scalable oversight. While numerous studies have been proposed to evaluate critique ability of LLMs, their comprehensiveness and reliability are still limited. To overcome this problem, we introduce CriticEval, a novel benchmark designed to comprehensively and reliably evaluate critique ability of LLMs. Specifically, to ensure the comprehensiveness, CriticEval evaluates critique ability from four dimensions across nine diverse task scenarios. It evaluates both scalar-valued and textual critiques, targeting responses of varying quality. To ensure the reliability, a large number of critiques are annotated to serve as references, enabling GPT-4 to evaluate textual critiques reliably. Extensive evaluations of open-source and closed-source LLMs first validate the reliability of evaluation in CriticEval. Then, experimental results demonstrate the promising potential of open-source LLMs, the effectiveness of critique datasets and several intriguing relationships between the critique ability and some critical factors, including task types, response qualities and critique dimensions.

==> sections/case_study.tex <==
%\vspace{-1.5cm}
\section{Case Study}

\subsection{Case Study on Subjective Evaluation}

In this subsection, we present a specific instance of subjective evaluation using the Qwen-72B-Chat model within the general chat domain. Further examples encompassing both objective and subjective assessments across varied critique tasks are detailed in Appendix \ref{sec:appendix_case_study}. The case is illustrated in Figure \ref{img:feedback_case_study}.
The case is shown in Figure \ref{img:feedback_case_study}.
In this case, the generated response contains factual errors `` cool music from 1920 are King of the Jazz Band and In the Mood.''. High-quality reference feedback points out these flaws, while Qwen-72B-Chat's feedback fails to find out these problems, leading to a low quality score 2 (1-10).

